The structure of mean equicontinuous group actions

We study mean equicontinuous actions of locally compact $\sigma$-compact amenable groups on compact metric spaces. In this setting, we establish the equivalence of mean equicontinuity and topo-isomorphy to the maximal equicontinuous factor and provide a characterization of mean equicontinuity of an action via properties of its product. This characterization enables us to show the equivalence of mean equicontinuity and the weaker notion of Besicovitch-mean equicontinuity in fairly high generality, including actions of abelian groups as well as minimal actions of general groups. In the minimal case, we further conclude that mean equicontinuity is equivalent to discrete spectrum with continuous eigenfunctions. Applications of our results yield a new class of non-abelian mean equicontinuous examples as well as a characterization of those extensions of mean equicontinuous actions which are still mean equicontinuous.

==> bibstandard.tex <==
%  Änderungen übertragen aus 
%  sna.tex (eV) sdic (vV 27.10.05)
%
%
%
%
%              für den Fall, dass doch \frac{\omega}{2} statt \omega als ``Frequenz'' des qp-Faktors benötigt wird
\newcommand{\w}{\omega}
\newcommand{\x}{x}
\newcommand{\faktor}{}
\newcommand{\fakt}{}

%
%		weitere vorübergehende Bez.
\newcommand{\X}{\ensuremath{X}}
\newcommand{\Sep}{\ensuremath{\operatorname{Sep}}}
\newcommand{\Span}{\ensuremath{\operatorname{Span}}}
% 
% 
% 
%
%
%
%		komplexe Zahlen
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
%
%
%		römische Ziffern
\newcommand{\RM}[1]{\MakeUppercase{\romannumeral #1}}
%
%
%		Skalarprodukt
\newcommand{\skp}[1]{\langle #1 \rangle}
%
%
%		Operatoren
\renewcommand{\d}{\ensuremath{\partial}}
\newcommand{\dw}{\ensuremath{\partial_\omega}}
\newcommand{\kom}[1]{\ensuremath{\left [ #1 \right ]}}
\newcommand{\tr}{\ensuremath{\operatorname{tr} }}
\newcommand{\id}{\ensuremath{\operatorname{id} }}
%		Matrizen
\newcommand{\mat}[4]{\ensuremath{\begin{pmatrix} #1 & #2 \\ #3 & #4\end{pmatrix}}}
\renewcommand{\vec}[2]{\ensuremath{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}}

%		Schriftarten
\newcommand{\mc}{\mathcal}

%               Listen
\newcommand{\alphlist}{\begin{list}{(\alph{enumi})}{\usecounter{enumi}}}
\newcommand{\romanlist}{\begin{list}{(\roman{enumi})}{\usecounter{enumi}}}
\newcommand{\listend}{\end{list}}

%               Symbole
\newcommand{\<}{\ensuremath{\stackrel{(\varepsilon_0)}{<}}}
\renewcommand{\:}{\colon}
\renewcommand{\=}{\coloneqq}
\newcommand{\ldot}{\ensuremath{\textbf{.}}}
\newcommand{\ld}{\ensuremath{,\ldots,}}
\newcommand{\ssq}{\ensuremath{\subseteq}}
\newcommand{\smin}{\ensuremath{\setminus}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\alp}{\ensuremath{\alpha}}
\newcommand{\lam}{\ensuremath{\lambda}}


%               Normen und Abstaende
\newcommand{\supnorm}[1]{\ensuremath{\parallel #1 \parallel_{\infty}}}
\newcommand{\einsnorm}[1]{\ensuremath{\parallel #1 \parallel_{1}}}
\newcommand{\zweinorm}[1]{\ensuremath{\parallel #1 \parallel_{2}}}
\newcommand{\pnorm}[1]{\ensuremath{\parallel #1 \parallel_{p}}}
\newcommand{\norm}[1]{\ensuremath{\parallel \! #1 \! \parallel}}
\newcommand{\rnorm}[1]{\ensuremath{\parallel #1 \parallel_{r}}}
\newcommand{\snorm}[1]{\ensuremath{\parallel #1 \parallel_{s}}}
\newcommand{\dist}[1]{\ensuremath{\operatorname{dist}\left( #1 \right)}}

%               Pfeile

\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\equi}{\ensuremath{\Leftrightarrow}}
\newcommand{\follows}{\ensuremath{\Rightarrow}}


%               Zahlenmengen

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\K}{\ensuremath{\mathbb{K}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}} 
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\renewcommand{\P}{\ensuremath{\mathbb{P}}}
\newcommand{\Proj}{\ensuremath{\mathbb{P}}}
  

%               Raeume

\newcommand{\kreis}{\ensuremath{\mathbb{T}^{1}}}
\newcommand{\ntorus}[1][2]{\ensuremath{\mathbb{T}^{#1}}}
\newcommand{\Rn}{\ensuremath{\mathbb{R}^{n}}}    
\newcommand{\Rd}{\ensuremath{\mathbb{R}^{d}}}    
\newcommand{\Rk}{\ensuremath{\mathbb{R}^{k}}}   
\renewcommand{\H}{\ensuremath{\mathscr H}}
\newcommand{\I}{\ensuremath{\mathcal I}}
\newcommand{\A}{\ensuremath{\mathcal A}}
\newcommand{\B}{\ensuremath{\mathcal B}}
%               Funktionenraeume
%\newcommand{\B}{\ensuremath{\mathscr B}}
\newcommand{\Br}{\ensuremath{\mathscr B_r}}
\newcommand{\Ceins}{\ensuremath{{\cal C}^{1}}}
\newcommand{\Leins}{\ensuremath{{\cal L}^{1}}}
\newcommand{\Leinsmu}{\ensuremath{{\cal L}^{1}_{\mu}}}
\newcommand{\Lpmu}{\ensuremath{{\cal L}^{p}_{\mu}}}
\newcommand{\Lzweimu}{\ensuremath{{\cal L}^{2}_{\mu}}}


%               Limiten
\newcommand{\nLim}{\ensuremath{\lim_{n\rightarrow\infty}}}
\newcommand{\iLim}{\ensuremath{\lim_{i\rightarrow\infty}}}
\newcommand{\jLim}{\ensuremath{\lim_{j\rightarrow\infty}}}
\newcommand{\kLim}{\ensuremath{\lim_{k\rightarrow\infty}}}

\newcommand{\xLim}{\ensuremath{\lim_{x\rightarrow\infty}}}
\newcommand{\yLim}{\ensuremath{\lim_{y\rightarrow\infty}}}
\newcommand{\sLim}{\ensuremath{\lim_{s\rightarrow\infty}}}
\newcommand{\rLim}{\ensuremath{\lim_{r\rightarrow\infty}}}
\newcommand{\tLim}{\ensuremath{\lim_{t\rightarrow\infty}}}
\newcommand{\hLim}{\ensuremath{\lim_{h\rightarrow\infty}}}
\newcommand{\aLim}{\ensuremath{\lim_{a\rightarrow\infty}}}

\newcommand{\xlim}{\ensuremath{\lim_{x\rightarrow 0}}}
\newcommand{\ylim}{\ensuremath{\lim_{y\rightarrow 0}}}

\newcommand{\rlim}{\ensuremath{\lim_{r\rightarrow 0}}}
\newcommand{\tlim}{\ensuremath{\lim_{t\rightarrow 0}}}
\newcommand{\hlim}{\ensuremath{\lim_{h\rightarrow 0}}}
\newcommand{\alim}{\ensuremath{\lim_{a\rightarrow 0}}}

\newcommand{\epslim}{\ensuremath{\lim_{\epsilon\rightarrow 0}}}
\newcommand{\dellim}{\ensuremath{\lim_{\delta\rightarrow 0}}}
\newcommand{\gamlim}{\ensuremath{\lim_{\gamma\rightarrow 0}}}


\newcommand{\nKonv}{\ensuremath{\stackrel{n\rightarrow
      \infty}{\longrightarrow}}}
\newcommand{\kKonv}{\ensuremath{\stackrel{k\rightarrow
      \infty}{\longrightarrow}}}
\newcommand{\pKonv}{\ensuremath{\stackrel{p\rightarrow
      \infty}{\longrightarrow}}}

\newcommand{\weakly}{\ensuremath{\stackrel{w.}{\rightarrow}}}
\newcommand{\slim}{\ensuremath{\operatorname{s}\!-\!\lim}}


%                  Folgenklammern
\newcommand{\nfolge}[1]{\ensuremath{(#1)_{n\in\mathbb{N}}}}
\newcommand{\kfolge}[1]{\ensuremath{(#1)_{k\in\mathbb{N}}}}
\newcommand{\ifolge}[1]{\ensuremath{(#1)_{i\in\mathbb{N}}}}
\newcommand{\jfolge}[1]{\ensuremath{(#1)_{j\in\mathbb{N}}}}
\newcommand{\mfolge}[1]{\ensuremath{(#1)_{m\in\mathbb{N}}}}
\newcommand{\lfolge}[1]{\ensuremath{(#1)_{l\in\mathbb{N}}}}
%
%
%
%
%		Familienklammern
\newcommand{\faml}[1]{\ensuremath{(#1_{\lambda})_{\lambda \in \Lambda}}}


%                       Anfang und Ende des Beweises 
\newcommand{\myqed}{{\raggedleft $\Box$ \\}}
\newcommand{\solidqed}{{\raggedleft \large $\blacksquare$ \\}}

\newcommand{\myproof}{\textit{Proof:}}
\newcommand{\bew}{\textit{Beweis:}}



%
%               Funktionen
%
\newcommand{\diam}{\ensuremath{\mathrm{diam}}}
\newcommand{\Id}{\ensuremath{\mathrm{Id}}}
\newcommand{\ind}{\ensuremath{\mathbf{1}}}
\newcommand{\sgn}{\ensuremath{\mathrm{sgn}}}
\newcommand{\supp}{\ensuremath{\mathrm{supp}}}
\newcommand{\graph}{\ensuremath{\mathrm{graph}}}
\newcommand{\artanh}{\ensuremath{\operatorname{artanh}}}
\newcommand{\fa}{\ensuremath{{f^\alpha}}}
\newcommand{\ga}{\ensuremath{{g^a}}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\Abs}[1]{\ensuremath{\left\|#1\right\|}}
\newcommand{\Leb}{\ensuremath{\operatorname{Leb}}}
%          Vereinigungen und Durchschnitte
\newcommand{\twoscriptcup}[2]{ \ensuremath{ \bigcup_{ \begin{array}{c}
\scriptstyle #1 \\  \scriptstyle #2 \end{array} }}}
\newcommand{\twoscriptuplus}[2]{ \ensuremath{\biguplus_{\begin{array}{c}
\scriptstyle #1 \\  \scriptstyle #2 \end{array} }}}
\newcommand{\twoscriptcap}[2]{ \ensuremath{\bigcap_{\begin{array}{c}
\scriptstyle #1 \\  \scriptstyle #2 \end{array} } }}


\newcommand{\icup}{\ensuremath{\bigcup_{i\in\N}}}
\newcommand{\jcup}{\ensuremath{\bigcup_{j\in\N}}}
\newcommand{\kcup}{\ensuremath{\bigcup_{k\in\N}}}
\newcommand{\lcup}{\ensuremath{\bigcup_{l\in\N}}}
\newcommand{\mcup}{\ensuremath{\bigcup_{m\in\N}}}
\newcommand{\ncup}{\ensuremath{\bigcup_{n\in\N}}}

\newcommand{\incup}{\ensuremath{\bigcup_{i=1}^n}}
\newcommand{\ikcup}{\ensuremath{\bigcup_{i=1}^k}}
\newcommand{\imcup}{\ensuremath{\bigcup_{i=1}^m}}
\newcommand{\ilcup}{\ensuremath{\bigcup_{i=1}^l}}
\newcommand{\ijcup}{\ensuremath{\bigcup_{i=1}^j}}

\newcommand{\jncup}{\ensuremath{\bigcup_{j=1}^n}}
\newcommand{\jkcup}{\ensuremath{\bigcup_{j=1}^k}}
\newcommand{\jmcup}{\ensuremath{\bigcup_{j=1}^m}}
\newcommand{\jlcup}{\ensuremath{\bigcup_{j=1}^l}}

\newcommand{\kncup}{\ensuremath{\bigcup_{k=1}^n}}
\newcommand{\kmcup}{\ensuremath{\bigcup_{k=1}^m}}
\newcommand{\klcup}{\ensuremath{\bigcup_{k=1}^l}}

\newcommand{\nmcup}{\ensuremath{\bigcup_{n=1}^m}}
\newcommand{\nkcup}{\ensuremath{\bigcup_{n=1}^k}}
\newcommand{\nlcup}{\ensuremath{\bigcup_{n=1}^l}}

\newcommand{\lkcup}{\ensuremath{\bigcup_{l=1}^k}}
\newcommand{\lmcup}{\ensuremath{\bigcup_{l=1}^m}}
\newcommand{\lncup}{\ensuremath{\bigcup_{l=1}^n}}
\newcommand{\licup}{\ensuremath{\bigcup_{l=1}^i}}
\newcommand{\ljcup}{\ensuremath{\bigcup_{l=1}^j}}



\newcommand{\icap}{\ensuremath{\bigcap_{i\in\N}}}
\newcommand{\jcap}{\ensuremath{\bigcap_{j\in\N}}}
\newcommand{\kcap}{\ensuremath{\bigcap_{k\in\N}}}
\newcommand{\lcap}{\ensuremath{\bigcap_{l\in\N}}}
\newcommand{\mcap}{\ensuremath{\bigcap_{m\in\N}}}
\newcommand{\ncap}{\ensuremath{\bigcap_{n\in\N}}}

\newcommand{\incap}{\ensuremath{\bigcap_{i=1}^n}}
\newcommand{\ikcap}{\ensuremath{\bigcap_{i=1}^k}}
\newcommand{\imcap}{\ensuremath{\bigcap_{i=1}^m}}
\newcommand{\ilcap}{\ensuremath{\bigcap_{i=1}^l}}
\newcommand{\ijcap}{\ensuremath{\bigcap_{i=1}^j}}

\newcommand{\jncap}{\ensuremath{\bigcap_{j=1}^n}}
\newcommand{\jkcap}{\ensuremath{\bigcap_{j=1}^k}}
\newcommand{\jmcap}{\ensuremath{\bigcap_{j=1}^m}}
\newcommand{\jlcap}{\ensuremath{\bigcap_{j=1}^l}}

\newcommand{\kncap}{\ensuremath{\bigcap_{k=1}^n}}
\newcommand{\kmcap}{\ensuremath{\bigcap_{k=1}^m}}
\newcommand{\klcap}{\ensuremath{\bigcap_{k=1}^l}}

\newcommand{\nmcap}{\ensuremath{\bigcap_{n=1}^m}}
\newcommand{\nkcap}{\ensuremath{\bigcap_{n=1}^k}}
\newcommand{\nlcap}{\ensuremath{\bigcap_{n=1}^l}}

\newcommand{\lkcap}{\ensuremath{\bigcap_{l=1}^k}}
\newcommand{\lmcap}{\ensuremath{\bigcap_{l=1}^m}}
\newcommand{\lncap}{\ensuremath{\bigcap_{l=1}^n}}
\newcommand{\licap}{\ensuremath{\bigcap_{l=1}^i}}
\newcommand{\ljcap}{\ensuremath{\bigcap_{l=1}^j}}



\newcommand{\iuplus}{\ensuremath{\biguplus_{i\in\N}}}
\newcommand{\juplus}{\ensuremath{\biguplus_{j\in\N}}}
\newcommand{\kuplus}{\ensuremath{\biguplus_{k\in\N}}}
\newcommand{\luplus}{\ensuremath{\biguplus_{l\in\N}}}
\newcommand{\muplus}{\ensuremath{\biguplus_{m\in\N}}}
\newcommand{\nuplus}{\ensuremath{\biguplus_{n\in\N}}}

\newcommand{\inuplus}{\ensuremath{\biguplus_{i=1}^n}}
\newcommand{\ikuplus}{\ensuremath{\biguplus_{i=1}^k}}
\newcommand{\imuplus}{\ensuremath{\biguplus_{i=1}^m}}
\newcommand{\iluplus}{\ensuremath{\biguplus_{i=1}^l}}
\newcommand{\ijuplus}{\ensuremath{\biguplus_{i=1}^j}}

\newcommand{\jnuplus}{\ensuremath{\biguplus_{j=1}^n}}
\newcommand{\jkuplus}{\ensuremath{\biguplus_{j=1}^k}}
\newcommand{\jmuplus}{\ensuremath{\biguplus_{j=1}^m}}
\newcommand{\jluplus}{\ensuremath{\biguplus_{j=1}^l}}

\newcommand{\knuplus}{\ensuremath{\biguplus_{k=1}^n}}
\newcommand{\kmuplus}{\ensuremath{\biguplus_{k=1}^m}}
\newcommand{\kluplus}{\ensuremath{\biguplus_{k=1}^l}}

\newcommand{\nmuplus}{\ensuremath{\biguplus_{n=1}^m}}
\newcommand{\nkuplus}{\ensuremath{\biguplus_{n=1}^k}}
\newcommand{\nluplus}{\ensuremath{\biguplus_{n=1}^l}}

\newcommand{\lkuplus}{\ensuremath{\biguplus_{l=1}^k}}
\newcommand{\lmuplus}{\ensuremath{\biguplus_{l=1}^m}}
\newcommand{\lnuplus}{\ensuremath{\biguplus_{l=1}^n}}
\newcommand{\liuplus}{\ensuremath{\biguplus_{l=1}^i}}
\newcommand{\ljuplus}{\ensuremath{\biguplus_{l=1}^j}}


\newcommand{\Icup}{\ensuremath{\bigcup_{i\in I}}}
\newcommand{\Icap}{\ensuremath{\bigcap_{i\in I}}}



%                 Summen

\newcommand{\twoscriptsum}[2]{ \ensuremath{\sum_{\begin{array}{c}
        \scriptstyle #1 \\ \scriptstyle #2 \end{array} }}}

\newcommand{\isum}{\ensuremath{\sum_{i\in\N}}}
\newcommand{\jsum}{\ensuremath{\sum_{j\in\N}}}
\newcommand{\ksum}{\ensuremath{\sum_{k\in\N}}}
\newcommand{\lsum}{\ensuremath{\sum_{l\in\N}}}
\newcommand{\msum}{\ensuremath{\sum_{m\in\N}}}
\newcommand{\nsum}{\ensuremath{\sum_{n\in\N}}}

\newcommand{\insum}{\ensuremath{\sum_{i=1}^n}}
\newcommand{\iksum}{\ensuremath{\sum_{i=1}^k}}
\newcommand{\imsum}{\ensuremath{\sum_{i=1}^m}}
\newcommand{\ilsum}{\ensuremath{\sum_{i=1}^l}}
\newcommand{\ijsum}{\ensuremath{\sum_{i=1}^j}}

\newcommand{\jnsum}{\ensuremath{\sum_{j=1}^n}}
\newcommand{\jksum}{\ensuremath{\sum_{j=1}^k}}
\newcommand{\jmsum}{\ensuremath{\sum_{j=1}^m}}
\newcommand{\jlsum}{\ensuremath{\sum_{j=1}^l}}

\newcommand{\knsum}{\ensuremath{\sum_{k=1}^n}}
\newcommand{\kmsum}{\ensuremath{\sum_{k=1}^m}}
\newcommand{\klsum}{\ensuremath{\sum_{k=1}^l}}

\newcommand{\nmsum}{\ensuremath{\sum_{n=1}^m}}
\newcommand{\nksum}{\ensuremath{\sum_{n=1}^k}}
\newcommand{\nlsum}{\ensuremath{\sum_{n=1}^l}}

\newcommand{\lksum}{\ensuremath{\sum_{l=1}^k}}
\newcommand{\lmsum}{\ensuremath{\sum_{l=1}^m}}
\newcommand{\lnsum}{\ensuremath{\sum_{l=1}^n}}
\newcommand{\lisum}{\ensuremath{\sum_{l=1}^i}}
\newcommand{\ljsum}{\ensuremath{\sum_{l=1}^j}}


\newcommand{\inergsum}{\ensuremath{\sum_{i=0}^{n-1}}}
\newcommand{\ikergsum}{\ensuremath{\sum_{i=0}^{k-1}}}
\newcommand{\imergsum}{\ensuremath{\sum_{i=0}^{m-1}}}
\newcommand{\ilergsum}{\ensuremath{\sum_{i=0}^{l-1}}}
\newcommand{\ijergsum}{\ensuremath{\sum_{i=0}^{j-1}}}

\newcommand{\jnergsum}{\ensuremath{\sum_{j=0}^{n-1}}}
\newcommand{\jkergsum}{\ensuremath{\sum_{j=0}^{k-1}}}
\newcommand{\jmergsum}{\ensuremath{\sum_{j=0}^{m-1}}}
\newcommand{\jlergsum}{\ensuremath{\sum_{j=0}^{l-1}}}

\newcommand{\knergsum}{\ensuremath{\sum_{k=0}^{n-1}}}
\newcommand{\kmergsum}{\ensuremath{\sum_{k=0}^{m-1}}}
\newcommand{\klergsum}{\ensuremath{\sum_{k=0}^{l-1}}}

\newcommand{\nmergsum}{\ensuremath{\sum_{n=0}^{m-1}}}
\newcommand{\nkergsum}{\ensuremath{\sum_{n=0}^{k-1}}}
\newcommand{\nlergsum}{\ensuremath{\sum_{n=0}^{l-1}}}

\newcommand{\lkergsum}{\ensuremath{\sum_{l=0}^{k-1}}}
\newcommand{\lmergsum}{\ensuremath{\sum_{l=0}^{m-1}}}
\newcommand{\lnergsum}{\ensuremath{\sum_{l=0}^{n-1}}}
\newcommand{\liergsum}{\ensuremath{\sum_{l=0}^{i-1}}}
\newcommand{\ljergsum}{\ensuremath{\sum_{l=0}^{j-1}}}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

